Relic Density of Axion Dark Matter in Standard and Non-Standard Cosmological Scenarios

In this master's thesis we study the production of axion dark matter through the so-called misalignment mechanism by considering that during that time, the universe was dominated by a new kind of fluid, different than radiation. We perform a very detailed analysis of the oscillation temperature and the relic density today, both analytically and numerically. Our findings show that on the one hand, the oscillation temperature is strongly influenced by the non-standard cosmology, affecting the relic density, and on the other hand, the energy density of the axion gets diluted, because the new fluid eventually decays, injecting entropy into the thermal bath. We find the predicted parameter space of axion dark matter for different non-standard cosmologies and we show its impact on the coupling of axions to two photons.

==> chapters/Archived.tex <==
\subsection{Anharmonicities}
As we have seen, the full cosine-potential of the axion makes the evolution equation of $\theta$ nonlinear, we have avoided this by considering a small $\theta$  such that the potential becomes approximately harmonic, namely $V (a) =m_a^2 a^2/2$ as we wrote in \cref{eq:rho_appr}. However, for large initial displacements $\theta_i \simeq \pi$, anharmonic corrections caused by axion
self-interactions become important \cite{Marsh:2015xka} and the potential becomes flatter than the used
potential, resulting in the axion field oscillations starting in a $R_{osc}$ delayed increasing
the relic abundance relative to the harmonic approximation. 






\subsection{Axion isocurvature}

If the axion field is already present during inflation, it will develop quantum fluctuations. There are
two kinds of such fluctuations, called the adiabatic fluctuations and the isocurvature fluctuations. The former are fluctuations in the total energy density $\delta \rho \neq 0$. While, the isocurvature fluctuations are characterized by the fixed total energy density $\delta \rho \neq 0$ and correspond to the type of fluctuations experienced by the axion field. In order to fix the energy density, the axion energy density needs to be compensated by the fluctuation in other fields \cite{hertzberg2008axion}, so for in a early universe we write
\be
\delta \rho_{iso}=0=\delta \rho_a+\sum \delta \rho_i +\delta \rho_r
\ee
where $\delta \rho_a$, $\delta \rho_i$ and $\delta \rho_r$ are the perturbations of the energy densities of axions,
other massive species and radiation, respectively. By \cref{eq:rhora} we know that $\delta\rho_r=4\rho_r\delta T/T$. Thinking that the rest of species become non-relativistic, we have  $\delta \rho_a=m_a\delta n_a$ and  $\delta \rho_i=m_i\delta n_i$, whit $n$ the number density. The amplitude of isocurvature fluctuations is characterized by the entropy quantity \cite{1990eaun}
\be
S=\frac{\delta(n/s)}{(n/s)}=\frac{\delta n}{n}-\frac{\delta s}{s}= \frac{\delta n}{n}-3\frac{\delta T}{T}
\label{eq:SS}
\ee
here $s$ is the entropy density and in last term in \cref{eq:SS} we have used \cref{eq:entropy}. The entropy quantity is zero for adiabatic species and non-zero for isocurvature species. 


In the early universe, we ignore the term $\delta T/T$, so for axions we can express $S_a$ just in terms of the misalignment angle $\theta$ as \cite{hertzberg2008axion,hamann2009isocurvature, Wantz:2009it}
\be
S_a\simeq \frac{\delta n_a}{n_a}=\frac{\theta^2-\langle \theta ^2 \rangle}{\langle \theta^2 \rangle}.
\ee
Now we can relate $S_a$ to the power spectrum of axion perturbations $\Delta_a^2(k)=\langle|S_a|^2\rangle$. In this point, keeping generality we consider that cold dark matter consists of axions and other particle but only axions contribute to isocurvature fluctuations, such that the amplitude of cold dark matter isocurvature fluctuations is given by \cite{beltran2007isocurvature}
\be
\Delta_S^2(k)=\left(\frac{\Omega_{a,0}}{\Omega_c}\right)^2 \Delta_a^2(k)= \left(\frac{\Omega_{a,0}}{\Omega_c}\right)^2 \frac{2 \sigma_\theta^2(\sigma_\theta^2+ 2\theta_i^2)}{(\theta_i^2+\sigma_\theta^2)^2}.
\label{eq:deltas}
\ee
In the previous expression we have assumed a Gaussian distribution and that mean value $\langle \theta \rangle=\theta_i$. Since  at  high temperatures the axion is massless, the misalignment angle fluctuations have variance \cite{Wantz:2009it}
\be
\sigma_\theta=\delta \left( \frac{a(x)}{f_a}\right)=\left( \frac{H_I}{2\pi f_a}\right)^2
\ee


Conventionally, the magnitude of isocurvature perturbations is parametrized as \cite{ade2016planck}
\be
\alpha(k_0)=\frac{\Delta_S^2(k_0)}{\Delta^2_\mathcal{R}(k_0)+\Delta^2_S(k_0)}
\label{eq:alfa1}
\ee
 here $k_0 = 0.002Mpc^{-1}$ is the pivot scale and  $\Delta^2_\mathcal{R}(k_0)$ is the amplitude of adiabatic fluctuations mentioned above which can be measured by CMB observations, $\Delta^2_\mathcal{R}(k_0) = 2.42\times 10^{-9}$ \cite{wmap2011seven}. Finally The adiabaticity $\alpha_(k_0)$ is constrained by the WMAP-7 + BAO + SN data to be \cite{wmap2011seven}
\be
\alpha(k_0) <0.077
\label{eq:alfa2}
\ee
it means that most of observed perturbations corresponds to adiabatic fluctuations. Plugging \cref{eq:alfa2} and $\Delta^2_\mathcal{R}(k_0)$ into  \cref{eq:alfa1} and then assuming that $\theta_i^2\gg \sigma_a^2$ in \cref{eq:deltas} \footnote{To consider $\theta_i^2\ll \sigma_a^2$ is inconsistent with the bound for $\alpha(k_0)$.} along with that axions give dominant contribution for cold dark matter abundance ($\Omega_{CDM} = \Omega_{a}$) we obtain a bound in the axion parameters given by
\be
H_I < 4.3\times 10^{-5} \theta_i f_a
\ee

==> chapters/biblio.tex <==
\begin{document}

\end{document}
